Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo

Riemannian manifold Hamiltonian (RMHMC) and Lagrangian Monte Carlo (LMC) have emerged as powerful methods of Bayesian inference. Unlike Euclidean Hamiltonian Monte Carlo (EHMC) and the Metropolis-adjusted Langevin algorithm (MALA), the geometric ergodicity of these Riemannian algorithms has not been extensively studied. On the other hand, the manifold Metropolis-adjusted Langevin algorithm (MMALA) has recently been shown to exhibit geometric ergodicity under certain conditions. This work investigates the mixture of the LMC and RMHMC transition kernels with MMALA in order to equip the resulting method with an "inherited" geometric ergodicity theory. We motivate this mixture kernel based on an analogy between single-step HMC and MALA. We then proceed to evaluate the original and modified transition kernels on several benchmark Bayesian inference tasks.

==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/appendices/proofs.tex <==
\section{Proofs}

\subsection{Proof of \Cref{geometric-ergodicity:prop:mala-hmc-equivalence}}\label{geometric-ergodicity:app:proof-mala-hmc-equivalence}

\begin{proof}
The proposal distribution of MALA is
\begin{align}
    \tilde{q}\vert q &\sim \mathrm{Normal}\paren{q + \frac{\epsilon^2}{2} \mathbf{A}^{-1}\nabla \log \pi(q), \epsilon^2 \mathbf{A}^{-1}} \\
    \tilde{\pi}(\tilde{q}\vert q) &\propto \exp\paren{-\frac{1}{2\epsilon^2} \paren{\tilde{q} - q - \frac{\epsilon^2}{2}\mathbf{A}^{-1} \nabla \log\pi(q)}^\top \mathbf{A} \paren{\tilde{q} - q - \frac{\epsilon^2}{2} \mathbf{A}^{-1} \nabla \log\pi(q)}} \\
    &= \exp\paren{-\frac{1}{2\epsilon^2} \paren{\mathbf{A}\tilde{q} - \mathbf{A}q - \frac{\epsilon^2}{2} \nabla \log\pi(q)}^\top \mathbf{A}^{-1} \paren{\mathbf{A}\tilde{q} - \mathbf{A}q - \frac{\epsilon^2}{2} \nabla \log\pi(q)}}.
\end{align}
Therefore, the acceptance probability of MALA is,
\begin{align}
\begin{split}
    \label{geometric-ergodicity:eq:mala-acceptance} &\min\set{1, \frac{\pi(\tilde{q}) \tilde{\pi}(q\vert \tilde{q})}{\pi(q) \tilde{\pi}(\tilde{q}\vert q)}} \\
    =& \min\set{1, \frac{\pi(\tilde{q})}{\pi(q)}\cdot \frac{\exp\paren{-\frac{1}{2\epsilon^2} \paren{\mathbf{A}q - \mathbf{A}\tilde{q} - \frac{\epsilon^2}{2} \nabla \log\pi(\tilde{q})}^\top \mathbf{A}^{-1} \paren{\mathbf{A}q - \mathbf{A}\tilde{q} - \frac{\epsilon^2}{2} \nabla \log\pi(\tilde{q})}}}{\exp\paren{-\frac{1}{2\epsilon^2} \paren{\mathbf{A}\tilde{q} - \mathbf{A}q - \frac{\epsilon^2}{2} \nabla \log\pi(q)}^\top \mathbf{A}^{-1} \paren{\mathbf{A}\tilde{q} - \mathbf{A}q - \frac{\epsilon^2}{2} \nabla \log\pi(q)}}}}.
\end{split}
\end{align}
The proposal $\tilde{q}$ given $q$ can be sampled by generating $z\sim\mathrm{Normal}(0, \mathrm{Id})$ and setting
\begin{align}
    \label{geometric-ergodicity:eq:mala-proposal} \tilde{q}=q+\frac{\epsilon}{2} \mathbf{A}^{-1}\nabla \log\pi(q) + \epsilon\sqrt{\mathbf{A}^{-1}} z.
\end{align}
In HMC, the leapfrog integrator is applied to the Hamiltonian $H(q, p) = -\log\pi(q) + \frac{1}{2} p^\top\mathbf{A}^{-1}p$. The sequence of updates is,
\begin{align}
    \bar{p} &= p + \frac{\epsilon}{2} \nabla\log\pi(q) \\
    \label{geometric-ergodicity:eq:hmc-proposal} \tilde{q}' &= q + \epsilon \mathbf{A}^{-1} \bar{p} \\
    &= q + \frac{\epsilon^2}{2}\mathbf{A}^{-1} \nabla \log \pi(q) + \epsilon \mathbf{A}^{-1} p \\
    \tilde{p}' &= \bar{p} + \frac{\epsilon}{2} \nabla\log\pi(\tilde{q}') \\
    &= p + \frac{\epsilon}{2} \nabla\log\pi(q) + \frac{\epsilon}{2} \nabla\log\pi(\tilde{q}').
\end{align}
When sampling from the distribution with density proportional to $\exp(-H(q, p))$, one sees by inspection that $p$ is independent of $q$ and that $p\sim\mathrm{Normal}(0, \mathbf{A})$. Therefore, using the same $z$ as in \cref{geometric-ergodicity:eq:mala-proposal}, we can sample $p$ by setting $p=\sqrt{\mathbf{A}} z$ so that $\epsilon\mathbf{A}^{-1} p = \epsilon\sqrt{\mathbf{A}^{-1}}z$; we therefore see that, in this case, HMC and MALA produce exactly the same proposal (i.e. $\tilde{q}'=\tilde{q}$). Recall that the HMC acceptance probability is,
\begin{align}
    \label{geometric-ergodicity:eq:hmc-acceptance} \min\set{1, \frac{\pi(\tilde{q})}{\pi(q)} \cdot \frac{\exp\paren{-\frac{1}{2} (\tilde{p}')^\top\mathbf{A}^{-1} (\tilde{p}')}}{\exp\paren{-\frac{1}{2} p^\top\mathbf{A}^{-1} p}}}.
\end{align}
By rearranging \cref{geometric-ergodicity:eq:hmc-proposal} we find,
\begin{align}
    p &= \frac{1}{\epsilon} \paren{\mathbf{A}\tilde{q} - \mathbf{A}q - \frac{\epsilon^2}{2} \nabla \log\pi(q)} \\
    \tilde{p}' &= \frac{1}{\epsilon} \paren{\mathbf{A}\tilde{q} - \mathbf{A}q + \frac{\epsilon^2}{2} \nabla\log\pi(\tilde{q})} \\
    &= -\frac{1}{\epsilon} \paren{\mathbf{A}q - \mathbf{A}\tilde{q} - \frac{\epsilon^2}{2} \nabla\log\pi(\tilde{q})}.
\end{align}
Substituting these into \cref{geometric-ergodicity:eq:hmc-acceptance} and comparing to \cref{geometric-ergodicity:eq:mala-acceptance} shows that not only are $\tilde{q}$ and $\tilde{q}'$ identical but that the acceptance probabilities are also identical. Therefore, the marginal chain of single-step HMC is exactly equivalent to the MALA chain.
\end{proof}

\subsection{Proof of \Cref{geometric-ergodicity:lem:marginal-transition-kernel}}\label{geometric-ergodicity:app:proof-marginal-transition-kernel}

\begin{proof}
  \begin{align}
      \mathrm{Pr}(q^{n+1}\in Q\vert q^n=q) &= \mathrm{Pr}(q^{n+1}\in Q ~\mathrm{and}~ p^{n+1}\in \R^m\vert q^n=q) \\
      &= \int_{\R^m} \mathrm{Pr}(q^{n+1}\in Q ~\mathrm{and}~ p^{n+1}\in \R^m\vert q^n=q, p^n=p) ~\pi(p\vert q)~\mathrm{d}p \\
      &= \int_{\R^m} K((q, p), (Q,\R^m)) ~\pi(p\vert q)~\mathrm{d}p.
  \end{align}
\end{proof}

\subsection{Proof of \Cref{geometric-ergodicity:prop:marginal-reversible}}\label{geometric-ergodicity:app:proof-marginal-reversible}

\begin{proof}
Given $Q, Q'\in\mathfrak{B}(\R^m)$ we have
\begin{align}
    \int_{Q} \tilde{K}(q, Q') ~\pi(q)~\mathrm{d}q &= \int_{Q} \int_{\R^m} K((q, p), (Q', \R^m)) ~\pi(p\vert q) ~\mathrm{d}p ~\pi(q)~\mathrm{d}q \\
    &= \int_{Q} \int_{\R^m} K((q, p), (Q', \R^m)) ~\pi(q, p) ~\mathrm{d}p ~\mathrm{d}q \\
    \label{geometric-ergodicity:eq:detailed-balance} &= \int_{Q'} \int_{\R^m} K((q, p), (Q, \R^m)) ~\pi(q, p) ~\mathrm{d}p ~\mathrm{d}q \\
    &= \int_{Q'} \int_{\R^m} K((q, p), (Q, \R^m)) ~\pi(p\vert q) ~\mathrm{d}p ~\pi(q)~\mathrm{d}q \\
    &= \int_{Q'} \tilde{K}(q, Q) ~\pi(q)~\mathrm{d}q,
\end{align}
where in \cref{geometric-ergodicity:eq:detailed-balance} we have used the fact that the phase space chain satisfies detailed balance with respect to $\pi(q, p)$. This verifies that the marginal chain satisfies detailed balance. 
\end{proof}

\subsection{Proof of Involution Composition}

\begin{proposition}\label{prop:involution-composition}
Suppose that $\Phi : \R^m\times\R^m\to\R^m\times\R^m$ is an invertible function and let $\mathbf{F}$ be the momentum flip function given in \cref{def:rmhmc-transition-kernel}. Suppose that $\mathbf{F}\circ\Phi$ is an involution, then $\mathbf{F}\circ\Phi^k$ is also an involution.
\end{proposition}
\begin{proof}
This will be proved by induction with the base case established by assumption. As the inductive hypothesis, assume that $\mathbf{F}\circ\Phi^k$ is an involution. Using the fact that $\mathbf{F}\circ \Phi$ is an involution, we immediately obtain that $\Phi^{-1}\circ\mathbf{F} = \mathbf{F}\circ\Phi$. Using the inductive hypothesis, one also has $\Phi^{-k}\circ\mathbf{F} = \mathbf{F}\circ\Phi^k$. Therefore, we obtain,
\begin{align}
    & \Phi^{-1}\circ\mathbf{F} = \mathbf{F}\circ\Phi \\
    \implies& \Phi^{-1}\circ\mathbf{F}\circ\Phi^k = \mathbf{F}\circ\Phi^{k+1} \\
    \implies& \Phi^{-1}\circ\Phi^{-k}\circ\mathbf{F} = \mathbf{F}\circ\Phi^{k+1} \\
    \implies& \Phi^{-k-1}\circ\mathbf{F} = \mathbf{F}\circ\Phi^{k+1} \\
    \implies& \mathbf{F}\circ\Phi^{k+1}\circ \mathbf{F}\circ\Phi^{k+1} = \mathrm{Id}.
\end{align}
This verifies that $\mathbf{F}\circ\Phi^{k+1}$ is also an involution.
\end{proof}



==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/figures/banana/ergodicity.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/ergodicity-mmd-euclidean.png}
    \caption{EHMC}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/ergodicity-mmd-riemannian.png}
    \caption{LMRMHMC}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/ergodicity-mmd-lagrange.png}
    \caption{LMLMC}
  \end{subfigure}
  \caption{We examine the ergodicity of the Markov chains as a function of the sampling step in the banana-shaped posterior distribution. We observe that the use of a smaller step-size degrades the ergodicity of the RMHMC, particularly when compared against the LMC algorithm. In both RMHMC and LMC, we observe that aggressively mixing with MMALA causes the Markov chain to mix more slowly; on the other hand, a relatively small mixing probability leads to ergodicity that is nearly indistinguishable from the unmodified implementations of RMHMC and LMC.}
  \label{geometric-ergodicity:fig:banana-ergodicity}
\end{figure}


==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/figures/banana/metrics.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/esjd.png}
    \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/min-ess.png}
    \caption{Min. ESS}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/min-ess-sec.png}
    \caption{Min. ESS / Sec.}
  \end{subfigure}
  \caption{We show the ESJD, the minimum ESS, and the time-normalized minimum ESS for inference in the banana-shaped posterior distribution. We observe that for both RMHMC and LMC, aggressively mixing with MMALA causes the ESJD distance to decrease; this correspondingly produces a decrease in the minimum ESS. For LMC, the time-normalized minimum ESS is a decreasing function of the mixing probability.}
  \label{geometric-ergodicity:fig:banana-metrics}
\end{figure}


==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/figures/cox-poisson/metrics.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/cox-poisson/esjd.png}
    \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/cox-poisson/min-ess.png}
    \caption{Min. ESS}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/cox-poisson/min-ess-sec.png}
    \caption{Min. ESS / Sec.}
  \end{subfigure}
  \caption{We show the ESJD, the minimum ESS, and the time-normalized minimum ESS for inference in the posterior distribution of the log-Gaussian Cox-Poisson model. For any mixing probability, the geometric methods enjoy larger time-normalized effective sample sizes than EHMC, with LMC outperforming RMHMC on these metrics. For nearly every mixing probability, we additionally observe that the ESJD is greater for LMC and RMHMC than for EHMC.}
  \label{geometric-ergodicity:fig:cox-poisson-metrics}
\end{figure}


==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/figures/fitzhugh-nagumo/ergodicity.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/ergodicity-mmd-euclidean.png}
    \caption{EHMC}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/ergodicity-mmd-riemannian.png}
    \caption{LMRMHMC}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/ergodicity-mmd-lagrange.png}
    \caption{LMLMC}
  \end{subfigure}
  \caption{We examine the ergodicity of the Markov chains as a function of the sampling step in the Fitzhugh-Nagumo posterior distribution. We observe that when a modest mixing probability is employed, the modified RMHMC and LMC transition kernels mix more efficiently than the EHMC transition kernel, being nearly indistinguishable from the unmodified RMHMC and LMC transition kernels. When one uses a large mixing probability, we see that the mixing rate is decreased.}
  \label{geometric-ergodicity:fig:fitzhugh-nagumo-ergodicity}
\end{figure}


==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/figures/fitzhugh-nagumo/metrics.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/esjd.png}
    \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/min-ess.png}
    \caption{Min. ESS}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/min-ess-sec.png}
    \caption{Min. ESS / Sec.}
  \end{subfigure}
  \caption{We show the ESJD, the minimum ESS, and the time-normalized minimum ESS for inference in the Fitzhugh-Nagumo posterior distribution. LMC dominates both RMHMC and EHMC in this inference task under the time-normalized ESS metrics with its greater computational expediency. When timing is not accounted for, we observe that RMHMC and LMC enjoy similar ESJD and minimum ESS metrics. We observe that for both RMHMC and LMC, aggressively mixing with MMALA causes the ESJD distance to decrease; this correspondingly produces a decrease in the minimum ESS.}
  \label{geometric-ergodicity:fig:fitzhugh-nagumo-metrics}
\end{figure}


==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/figures/logistic/metrics.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/logistic/esjd.png}
    \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/logistic/min-ess.png}
    \caption{Min. ESS}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/logistic/min-ess-sec.png}
    \caption{Min. ESS / Sec.}
  \end{subfigure}
  \caption{We show the ESJD, the minimum ESS, and the time-normalized minimum ESS for inference in the hierarchical Bayesian logistic regression posterior distribution. We observe that both of the geometric methods do not perform as well as standard HMC in this inference task. For each mixing weight with MMALA, we observe that RMHMC enjoys a greater ESJD and minimum ESS when compared against LMC; however, as LMC is a more computationally expedient procedure, LMC has a greater time-normalized ESS. In all of these metrics, however, EHMC dominates the geometric inference algorithms.}
  \label{geometric-ergodicity:fig:logistic-metrics}
\end{figure}


==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/figures/neal-funnel/ergodicity.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/ergodicity-mmd-euclidean.png}
    \caption{EHMC}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/ergodicity-mmd-riemannian.png}
    \caption{LMRMHMC}
  \end{subfigure}
  \caption{We examine the ergodicity of the Markov chains as a function of the sampling step in Neal's funnel distribution. We observe that EHMC struggles in this distribution due to the multiple spatial scales inherent in the funnel-shaped distribution. Moreover, we observe that aggressively mixing RMHMC with SMALA causes convergence in MMD to become increasingly slow, with convergence of the pure SMALA algorithm being slower than EHMC. On the other hand, a modest amount of mixing with SMALA produces ergodicity that is nearly indistinguishable from the unmodified implementation of RMHMC.}
  \label{geometric-ergodicity:fig:neal-funnel-ergodicity}
\end{figure}


==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/figures/neal-funnel/metrics.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/esjd.png}
    \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/ks.png}
    \caption{KS}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/min-ess-sec.png}
    \caption{Min. ESS / Sec.}
  \end{subfigure}
  \caption{We show the ESJD, the distribution of Kolmogorov-Smirnov statistics, and the time-normalized minimum ESS for inference in Neal's funnel distribution. Although RMHMC and EHMC have comparable time-normalized ESS, it is clear from the distribution of KS statistics that RMHMC produces samples that are closer to the target distribution in EHMC.}
  \label{geometric-ergodicity:fig:neal-funnel-metrics}
\end{figure}


==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/figures/stochastic-volatility/metrics.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/stochastic-volatility/esjd.png}
    \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/stochastic-volatility/min-ess.png}
    \caption{Min. ESS}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/stochastic-volatility/min-ess-sec.png}
    \caption{Min. ESS / Sec.}
  \end{subfigure}
  \caption{We show the ESJD, the minimum ESS, and the time-normalized minimum ESS for inference in the posterior distribution of the stochastic volatility model. We observe that both of the geometric methods with a modest mixing probability with MMALA produce time-normalized ESS that are competitive with EHMC. For each mixing weight with MMALA, we observe that LMC enjoys a greater ESJD when compared against RMHMC.}
  \label{geometric-ergodicity:fig:stochastic-volatility-metrics}
\end{figure}


==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/figures/t/ergodicity.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/ergodicity-mmd-euclidean.png}
    \caption{EHMC}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/ergodicity-mmd-riemannian.png}
    \caption{LMRMHMC}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/ergodicity-mmd-lagrange.png}
    \caption{LMLMC}
  \end{subfigure}
  \caption{We examine the ergodicity of the Markov chains as a function of the sampling step in the multiscale Student-$t$ distribution. Here we see that, in the case of LMC, it is beneficial from an ergodicity perspective to mix heavily with MMALA, whereas for RMHMC, only modest mixing probabilities can produce a modified Markov chain that is competitive with the unmodified version. The Euclidean HMC struggles in this posterior distribution due to the multiple spatial scales.}
  \label{geometric-ergodicity:fig:t-ergodicity}
\end{figure}


==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/figures/t/jump.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/esjd.png}
    \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/msjd.png}
    \caption{MSJD}
  \end{subfigure}
  \caption{We show the ESJD and the MSJD for inference in the multiscale Student-$t$ distribution. Curiously, EHMC enjoys the largest ESJD, but this does not correspond to more efficient sampling, as shown in the inferior distribution of KS statistics. To examine this property further, we also measured the MSJD, which reveals that EHMC is less effective in traversing the parameter space compared to the RMHMC geometric method.}
  \label{geometric-ergodicity:fig:t-jump}
\end{figure}


==> Geometric Ergodicity in Modified Variations of Riemannian Manifold and Lagrangian Monte Carlo/figures/t/metrics.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/ks.png}
    \caption{KS}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/min-ess-sec.png}
    \caption{Min. ESS / Sec.}
  \end{subfigure}
  \caption{We show the distribution of Kolmogorov-Smirnov statistics and the time-normalized minimum ESS for inference in the multiscale Student-$t$ distribution. For the geometric methods, we observe that RMHMC has much larger ESJD than LMC; however, in terms of time-normalized performance, it is best to fully mix either method with MMALA. Indeed, we find that MMALA on its own produces a distribution of KS statistics that is competitive with any of the mixture kernels.}
  \label{geometric-ergodicity:fig:t-metrics}
\end{figure}

